The causality between the rapid rotation of a sunspot and an X3.4 flare

Using multi-wavelength data of Hinode, a rapid rotation of a sunspot in active region NOAA 10930 is studied in detail. We found the extra-ordinary counterclockwise rotation of the sunspot with positive polarity before an X3.4 flare. From a series of vector magnetograms, it is found that the magnetic force lines highly sheared along the neutral line accompanying the sunspot rotation. Furthermore, it is also found that the sheared loops and an inverse S-shaped magnetic loop in the corona formed gradually after the sunspot rotation. The X3.4 flare can be reasonably regarded as a result of this movement. The detailed analysis provides an evidence that sunspot rotation leads to magnetic field lines twisting in the photosphere, the twist is then transported into the corona, and finally flares are triggered.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
graphicx.sty   ---- a new package for embodying graphics, for LaTeX2e  
psfig.sty      ---- a package for graphics inclusion  
epsf.sty       ---- another package for graphics inclusion  
natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
f?.eps         ---- three demo figures used in the LaTeX template source

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org


